Busy beavers gone wild

We show some incompleteness results a la Chaitin using the busy beaver functions. Then, with the help of ordinal logics, we show how to obtain a theory in which the values of the busy beaver functions can be provably established and use this to reveal a structure on the provability of the values of these functions.

==> eptcsdata.tex <==
\providecommand{\eid}{12}

